Long-term instability of the inner Solar System: numerical experiments

Apart from being chaotic, the inner planets in the Solar System constitute an open system, as they are forced by the regular long-term motion of the outer ones. No integrals of motion can bound a priori the stochastic wanderings in their high-dimensional phase space. Still, the probability of a dynamical instability is remarkably low over the next 5 billion years, a timescale thousand times longer than the Lyapunov time. The dynamical half-life of Mercury has indeed been estimated recently at 40 billion years. By means of the computer algebra system TRIP, we consider a set of dynamical models resulting from truncation of the forced secular dynamics recently proposed for the inner planets at different degrees in eccentricities and inclinations. Through ensembles of $10^3$ to $10^5$ numerical integrations spanning 5 to 100 Gyr, we find that the Hamiltonian truncated at degree 4 practically does not allow any instability over 5 Gyr. The destabilisation is mainly due to terms of degree 6. This surprising result suggests an analogy to the Fermi-Pasta-Ulam-Tsingou problem, in which tangency to Toda Hamiltonian explains the very long timescale of thermalisation, which Fermi unsuccessfully looked for.

==> new_commands.tex <==
% Format statistical results with their bounds
\makeatletter
\newcommand{\raisemath}[1]{\mathpalette{\raiseboxmath{#1}}}
\newcommand{\raiseboxmath}[3]{\raisebox{#1}{$#2#3$}}
\makeatother
\newcommand{\stats}[3]{${#1}_{\raisemath{2pt}{\scriptscriptstyle #2}}^{\raisemath{0.5pt}{\scriptscriptstyle #3}}$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\g@addto@macro{\endtabular}{\rowfont{}}% Clear row font
\makeatother
\newcommand{\rowfonttype}{}% Current row font
\newcommand{\rowfont}[1]{% Set current row font
   \gdef\rowfonttype{#1}#1%
}
\newcolumntype{L}{>{\rowfonttype}l}

% Please keep new commands to a minimum, and use \newcommand not \def to avoid
% overwriting existing commands. Example:
%\newcommand{\pcm}{\,cm$^{-2}$}	% per cm-squared
\newcommand{\Poincare}{Poincar\'{e}}
\newcommand{\arcsecyr}{$^{\prime\prime} \,{\textrm{yr}}^{-1}$}
\newcommand{\arcsecyrtext}{${\textrm{arcsec yr}}^{-1}$}

\let\vec\boldsymbol
\def\E{\mathrm{E}}
\def\inc{\mathcal{I}}

\def\DOF{DOF}
\newcommand{\nomsol}{$\mathcal{S}$}
\newcommand{\lienomsol}{$\mathcal{S}^\prime$}
% Format statistical results with their bounds

\newcommand{\subscript}[2]{#1_{\textnormal{\scriptsize #2}}}
\newcommand{\superscript}[2]{#1^{\textnormal{\scriptsize #2}}}

\newcommand{\Hsec}{\widehat{H}}
\newcommand{\Hiss}{\mathcal{H}}
\newcommand{\HLL}{\subscript{\Hsec}{LL}}

\newcommand{\inn}[1]{\subscript{#1}{i}}
\newcommand{\out}[1]{\subscript{#1}{o}}

\newcommand{\gLL}{\subscript{g}{LL}}
\newcommand{\sLL}{\subscript{s}{LL}}
\newcommand{\vecomegaLL}{\subscript{\vec{\omega}}{LL}}

\newcommand{\vecu}{\vec{u}}
\newcommand{\vecv}{\vec{v}}

\newcommand{\Huv}{\mathbb{H}}

\newcommand{\Chi}{X}
\newcommand{\vecChi}{\vec{\Chi}}
\newcommand{\vecchi}{\vec{\chi}}
\newcommand{\vecPsi}{\vec{\Psi}}
\newcommand{\vecpsi}{\vec{\psi}}
\newcommand{\vecI}{\vec{I}}
\newcommand{\vectheta}{\vec{\theta}}
\newcommand{\veck}{\vec{k}}
\newcommand{\vecl}{\vec{\ell}}

\newcommand{\vecomegamean}{\overline{\vec{\omega}}}
\newcommand{\vecomegaout}{\out{\vec{\omega}}}

\newcommand{\fourcoeff}[3]{\widetilde{\Huv}_{#1}^{\vec{#2},\vec{#3}}}
\newcommand{\Ham}[1]{\Huv_{#1}}
\newcommand{\Hamstar}[1]{\Huv_{#1}^\star}
\newcommand{\lieham}{\Huv^\prime}
\newcommand{\Hamstart}{\Ham{6}}

\newcommand{\lieI}{\vecI^\prime}
\newcommand{\lietheta}{\vectheta^\prime}
\newcommand{\liePhi}{\vec{\Phi}^\prime}
\newcommand{\liephi}{\vec{\phi}^\prime}
\newcommand{\lieomega}{\vec{\omega}^\prime}
\newcommand{\lieomegamean}{\vec{\vecomegamean}^\prime}

\newcommand{\liefourcoeff}[2]{\widetilde{\Huv}_{2n}^{\prime \, \vec{#1},\vec{#2}}}

\newcommand{\vecp}{\vec{p}}
\newcommand{\vecvarphi}{\vec{\varphi}}
\newcommand{\matM}{\mathbb{M}}
\newcommand{\vece}{\vec{e}}

\newcommand{\conj}[1]{\overline{#1}}
\newcommand{\lieChi}{\vec{\Chi}^\prime}
\newcommand{\liePsi}{\vec{\Psi}^\prime}

\def\F{\mathcal{F}}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}

\newcommand{\lietransf}{\mathcal{L}}

\def\omegaell{\omega_\mathrm{ell}}
\def\omegahyp{\omega_\mathrm{hyp}}
\def\halfwidth{\Delta\overline{\omega}}
\def\omegamean{\overline{\omega}}


\DeclareMathOperator*{\argmax}{arg\,max}

